A Simple Baseline with Single-encoder for Referring Image Segmentation

Referring image segmentation (RIS) requires dense vision-language interactions between visual pixels and textual words to segment objects based on a given description. However, commonly adapted dual-encoders in RIS, e.g., Swin transformer and BERT (uni-modal encoders) or CLIP (a multi-modal dual-encoder), lack dense multi-modal interactions during pre-training, leading to a gap with a pixel-level RIS task. To bridge this gap, existing RIS methods often rely on multi-modal fusion modules that interact two encoders, but this approach leads to high computational costs. In this paper, we present a novel RIS method with a single-encoder, i.e., BEiT-3, maximizing the potential of shared self-attention across all framework components. This enables seamless interactions of two modalities from input to final prediction, producing granularly aligned multi-modal features. Furthermore, we propose lightweight yet effective decoder modules, a Shared FPN and a Shared Mask Decoder, which contribute to the high efficiency of our model. Our simple baseline with a single encoder achieves outstanding performances on the RIS benchmark datasets while maintaining computational efficiency, compared to the most recent SoTA methods based on dual-encoders.

==> tables/others.tex <==
\begin{table}[]
    \centering
    \caption{\sh{Others on Flawless}}
    \begin{tabular}{c|ccc}
    \hline
    Backbones     & RefCOCO & RefCOCO+ &  RefCOCOg  \\ \hline
    CLIP (w/Flawless)     & & & \\
    SWin-B (w/Flawless) & & & \\ \cdashline{1-4}[1pt/1pt]
    BEiT-3 (w/Flawless) & & & \\
    \hline
    \end{tabular}
    \label{tab:my_label}
\end{table}
